A Protection Method in Active Distribution Grids with High Penetration of Renewable Energy Sources

A protection method in active distribution networks is proposed in this paper. In active distribution systems, fault currents flow in multiple directions and presents a varying range of value, which poses a great challenge of maintaining coordination among protective devices on feeders. The proposed protection method addresses this challenge by simultaneously adjusting DG's output power and protection devices' settings in pre-fault networks. Comparing to previous protection solutions, the proposed method considers the influences from renewable DG's intermittency, and explores the economic and protection benefits of DG's active participation. The formulation of proposed method is decomposed into two optimization sub-problems, coupling through the constraint on fuse-recloser coordination. This decomposed mathematical structure effectively extinguishes the non-linearity arising from reclosers' time-current inverse characteristics, and greatly reduces computation efforts.

==> section2_1.tex <==
Conventional distribution grids are radial in nature, so that faults can be isolated conveniently from its upstream networks. Fig.~\ref{fig: Fig2} shows a typical protection configuration. Before DG's integration, fault current is fed from the single source and decreases along the feeder, flowing to the fault location \textcolor{red}{cite}. Because fault location and severity can be implied from current magnitudes, Over-Current (OC) scheme is deployed to protect the network. The main feeders are protected by reclosers and relays. A distribution network are usually equipped a few reclosers along the feeders, and one relay at the head of the feeders. Along a main feeder, three-phase, two-phase and single-phase laterals are tapped to supply loads. Laterals are protected by fuses. Under distribution automation, some laterals are installed with reclosers (referred in industry as ``trip savers'')\textcolor{red}{cite}. However, the large number of laterals and high cost of lateral reclosers make the fuses, which have much lower cost and less application complicacy, still the top choice for lateral protection. 

\begin{figure}[!t]
\centering
\includegraphics[width=0.48\textwidth]{Fig2}
\caption{Protection configuration of a LV network.}
\label{fig: Fig2}
\vspace{-4mm}
\end{figure}

On the occurrence of a fault, if the primary protective device always picks up before the backup devices, and the backup devices pick up within a required time in case the primary device subject to a failure, then the protection system is said coordinated. For feeder protection, coordination is required among (i) fuse-fuse; (ii) fuse-recloser, (iii) recloser-recloser. The last category includes recloser-relay. 

Protection coordination directly affects system reliability. ~\ref{fig:Fig2} shows two examples. For a fault happens at A, if coordination is lost between two fuses, F1 and F2, F1 will clear the fault before F2, and more customers will be interrupted than necessary. For a temporary fault happens at B, if coordination is lost between a recloser and a fuse, R1 and F3, F3 will blow before R1 trips. Because replacing the fuse is likely to take longer time than reclosing, this loss of coordination converts a temporary fault to permanent fault. The first example results in greater Energy Not Supplied (ENS), and the second results in greater System Average Interruption Duration Index (SAIDI).     

Two concepts to define coordination performance are \it{coordination range} and \it{coordination margin}. For the  
\subsection{protection coordination requirements}

These overcurrent devices operate coordinately to clear faults. Over 95\% of faults in distribution networks are temporary and can be cleared through reclosers. When permanent faults occur, opening reclosers for a preset timeframe will not clear the faults, fuses are melt to isolate the laterals. Once a fuse picks up a fault, it cannot be used again. Replacement of used fuses generates cost \cite{anderson}. Therefore, the coordination between fuses and reclosers are stated by the rule of economics. Namely, once a fault is detected, reclosers should operate first, if the fault is not cleared and appears to be permanent, then fuses are ``consumed'' to take the faulted lateral away. For faults happen on the primary feeder and are not temporary, the CB at the substation side is operated to clear the fault by de-energizing the whole feeder. A CB is also likely to have higher operation rating than reclosers, and operates at occurrence of serious faults that cannot be cleared by reclosers.

Coordination between reclosers is realized by setting their responding time. To minimize areas of service interruption, the recloser at the nearest upstream to the fault operates first, if fails, then is backup by its next upstream recloser. The Time-Current (TC) characteristics of overcurrent reclosers can be classified, by inverse level, as definite, inverse, very inverse, and extremely inverse, depicted in Fig.~\ref{fig: Fig3}. While the definite time reclosers have an almost constant time of response for any current exceeding about 10 times minimum pickup, the extremely inverse reclosers trip much faster at a high fault current. The inverse and very inverse performance are in between. 


\begin{figure}[!t]
\centering
\includegraphics[width=0.5\textwidth]{Fig3}
\caption{Time-Current (TC) inverse characteristics of overcurrent reclosers.}
\label{fig: Fig3}
\vspace{-4mm}
\end{figure}

These TC characteristics make the definite time reclosers a good choice for LV networks connected with DG, which intermittency results in a large difference of fault current at its maximum and minimum. However, extreme inverse reclosers display much better features of coordination margins between adjacent reclosers and fuses, especially when there is a considerable drop in fault current from one recloser location to the next, which is often observed in the DG-connected LV networks. Using adaptive reclosers can resolve this choice dilemma: reclosers' Time-Dial Settings (TDS) are adapted to detect fault currents at varying DG's output, in the meanwhile, more inverse TC characteristics are adopted for higher selectivity.




==> submission pdf latex/conclusion.tex <==
Legacy protection system at distribution level assumes power flowing in single direction from the substation. Increasing penetration of Distributed Generation (DG) invalidates this assumption and will disrupt protection coordination. Solutions proposed in previous studies include (i) limiting DG's fault current contribution; (ii) deploying microprocessor-based recloser/relays; and (iii) deploying non-overcurrent protection schemes. Deficiencies of these solutions can be attributed to their high cost, inflexibility of implementation, and limited effectiveness under high penetration of renewable DG.

To retrieve protection coordination in active distribution grids, this paper proposes a protection method which integrally adjusts the settings of protection devices and DG's output in pre-fault distribution networks. The formulation of the proposed method is decomposed into two optimization problems, aiming at two distinct objectives: maximizing total power output from DG's, and retaining protection coordination and sensitivity. This decomposed mathematical structure embodies the following benefits: (i) reducing computation effort by extinguishing the non-linearity of relay/reclosers' time-current inverse characteristics; (ii) enabling adaptive protection and DG control under different timeframes; (iii) providing implementation flexibility based on available communication and automation level of distribution grids. These benefits are demonstrated through numerical cases on the IEEE-37 bus system. 
 



==> submission pdf latex/section1.tex <==
\noindent {\bf{\it Variables}}
%\noindent \begin{tabular}{l p{7cm}}
\begin{labeling}{alligator}
%\begin{itemize}
\item [$I^f_P, I^f_B$]  fault current seen by the primary and backup protective device,
%\item [$I^f_B$]  fault current seen by the backup protective device,
%${\Delta} I^f$ fault current disparity seen by the backup device,\\
\item [$\Delta I^f_{FR,j}$] fault current disparity between recloser at node $j$ and its lateral fuse,
\item [${\Delta} I^f_{RR,j}$] fault current disparity between the primary recloser at node $j$ and its backup recloser $j-1$,
\item [$I^f_{max}, I^f_{min}$]  maximum and minimum fault current,
%\item [$I^f_{max}$] maximum fault current,
\item [$I^f_{R,j}$] fault current seen by the recolser at node $j$,
\item [$I^f_{F,i}$] fault current seen by the fuse at lateral $i$,
\item [$I^f_{G,i}$] fault current contributed by DG connected at lateral $i$,
\item [$P_i,Q_i$] real and reactive power flowing on the feeder section between lateral $i$ and lateral $i+1$ ,
%\item [$Q_i$] reactive power flowing on the feeder section between lateral $i$ and lateral $i+1$,
\item [$P_{D,i},Q_{D,i}$] total real and reactive power demand of all loads on lateral $i$,
%\item [$Q_{D,i}$] total reactive power demand of all loads on lateral $i$,
\item [$P_{G,i},Q_{G,i}$] real and reactive power output from DG at lateral $i$,
%\item [$Q_{G,i}$] reactive power output from DG at lateral $i$,
\item [$V_i$] terminal voltage magnitude of lateral $i$,
%\end{itemize}
\end{labeling}
\vspace{2mm}
\noindent {\bf{\it Functions}}
%\noindent \begin{tabular}{l p{7cm}}
%$T(\cdot)$ & time inverse function of a protective device,\\
\begin{labeling}{alligator}
\item[$T_{R,j}$] Time-Current Inverse (TCI) curve of recloser $j$,
\item[$T_P, T_B$] response time of the primary and backup protective device, which is calculated by the TCI curve $T_P(I^f_P)$ and $T_B(I^f_B)$ .
%\item[$T_B$] response time of the secondary protective device.
\end{labeling}

\vspace{2mm}
\noindent {\bf{\it Parameters}}
%\noindent \begin{tabular}{l p{7cm}}
\begin{labeling}{alligator}
\item[$r_i,x_i$]  resistance and reactance of the feeder section between lateral $i$ and $i+1$,
%\item[$x_i$] reactance of the feeder section between lateral $i$ and $i+1$,
%\item[${\Delta} T_$] coordination margin between the primary device and backup device,
\item[${\Delta}T_{FR}$] coordination margin between the recloser and its lateral fuse,
\item[${\Delta}T_{RR}$]  coordination margin between two reclosers.
\item[$D_{R,j}$] time dial setting of recloser $j$,
\item[$I^p_{R,j}$] pickup current of recloser $j$,
\end{labeling}

\vspace{2mm}
\noindent {\bf{\it Sets}}
\begin{labeling}{alligator}
\item[$\mathcal{J}$] bus/nodes on the main feeder,
\item[$\mathcal{I}$] laterals and DG inter-ties tapped on the main feeder,
\item[$\mathcal{I}^{j}$] laterals tapped on the feeder section between node $j$ and $j+1$,
\item[$\mathcal{I}^u_{j},\mathcal{I}^d_{j}$] laterals upstream and downstream to node $j$,   
%\item[$\mathcal{I}^d_{j}$] laterals downstream to node $j$
\end{labeling}

==> submission pdf latex/section2.tex <==
Conventional distribution grids are radial in nature, so that faults can be isolated conveniently from its upstream networks. Fig.~\ref{fig: Fig1} shows a typical protection configuration. Before DG's integration, fault current is fed from a single source and decreases along the feeder, flowing to the fault location \cite{Barker}.  
%Because fault location and severity can be implied from current magnitudes, Over-Current (OC) scheme is deployed to protect the network.
The main feeders are protected by reclosers and relays. A distribution network usually installs a few reclosers along the feeders, and one relay at the head of each feeders. Along a main feeder, laterals are tapped to supply loads. Laterals are protected by fuses. With distribution system becomes more automated, some laterals are installed with reclosers \cite{Fumilayo}. However, the large number of laterals and high cost of lateral reclosers make the fuses, which have much lower cost and much less application complicacy, the top choice for lateral protection. 
%
%\begin{figure}[!t]
%\centering
%\includegraphics[width=0.48\textwidth]{Fig2}
%\caption{Protection configuration of a distribution network.}
%\label{fig: Fig2}
%\vspace{-4mm}
%\end{figure}
\vspace{-2mm}
\subsection{Protection coordination requirements}
Protection coordination directly affects system reliability. For feeders' protection, coordination is required among (i) fuse-fuse; (ii) fuse-recloser, and (iii) recloser-recloser. The last category includes recloser-relay. During the restoration post-fault, coordination may be required among protective devices of feeders , loads (primarily induction motors) and DG's reclosers \cite{anderson, Kersting}. In this paper, we restrict the discussion to the pre-fault and fault clearing process.
%~\ref{fig:Fig2} shows two examples. For a fault happens at A, if coordination is lost between two fuses ($F1$ and $F2$), $F1$ will clear the fault before $F2$, and more customers will be interrupted than necessary. For a temporary fault happens at B, if coordination is lost between a recloser and a fuse ($R1$ and $F3$), $F3$ will blow before $R1$ trips. Because replacing the fuse is likely to take longer time than reclosing, this loss of coordination converts a temporary fault to permanent fault. The first example results in greater Energy Not Supplied (ENS), and the second results in greater System Average Interruption Duration Index (SAIDI).     

Two concepts defining coordination performance are {\it coordination range} and {\it coordination margin}. A pair of protective devices must be coordinated for all the fault currents within $I^f_{min}$ and $I^f_{max}$. This range of current is called the coordination range \cite{Girgis}. A time margin must be preserved for the response time between the primary and backup protective devices . This time is called coordination margin \cite{anderson}. Mathematically, the primary and backup devices are coordinated if and only if,
%\begin{equation}
% \left.\begin{aligned}\label{cod_range}
%    T_P(I^f_{min})\leq T_B(I^f_{min})\\
%       T_P(I^f_{max})\leq T_B(I^f_{max})
%       \end{aligned}
% \right\}
% \forall I^f_B, I^f_P\in [I^f_{min},I^f_{max}]
%\end{equation}

\begin{align} \label{cod_range}
\begin{split}
  T_P(I^f_{min})\leq T_B(I^f_{min})\\
       T_P(I^f_{max})\leq T_B(I^f_{max})
\end{split}
\end{align}  
and 
\begin{equation} \label{cod_margin}
T_B(I^f_B) - T_P(I^f_P)  \geq \Delta T; \forall I^f_B, I^f_P\in [I^f_{min},I^f_{max}]
\end{equation} 

Fig.~\ref{fig: fr1} and Fig.~\ref{fig: rr1} illustrates the coordination range for fuse-recloser and recloser-recloser. In a passive distribution system (i.e. before DG's integration), the primary and backup devices see the same fault current, $I^f_P = I^f_B$.  

\begin{figure}[t!]
\vspace{-4mm}
\setlength{\abovecaptionskip}{-3 pt}
\hspace*{-6mm}
\includegraphics[width=0.53\textwidth]{fr1}
\centering
\caption{Coordination margin and coordination range for a recloser and its lateral fuse. The reclosing sequence is fast-fast-slow.}
\label{fig: fr1}
\vspace{-4mm}
\end{figure}


\begin{figure}[t!]
\vspace{-4mm}
\setlength{\abovecaptionskip}{-10 pt}
\hspace*{-6mm}
\includegraphics[width=0.52\textwidth]{rr1}
\centering
\caption{Backup delay increasing due to DG's installation. The backup response delay is $(T_{R,j}-T_{R,(j+1)})^0$ before DG's installation, and increases to $(T_{R,j}-T_{R,(j+1)})^1$ after DG units connected to the feeder section between node $j$ and $j+1$. The two reclosers see different fault currents after DG's installation.}
\label{fig: rr1}
\vspace{-4mm}
\end{figure}

The coordination for fuse-fuse and recloser-recloser follows the principle that upstream devices backup downstream devices. In distribution grids, $70\%-95\%$ faults are temporary faults and can be cleared by reclosing operation \cite{glover2011power, Kersting, ieee2004impact}. Relays are used to clear up the permanent faults that cannot be cleared by downstream reclosers and backup for all protective devices on feeders.

The recloser-fuse coordination scheme varies by utilities' practice. Basically, two coordination schemes are deployed, fuse saving and fuse sacrificing  \cite{ieee2004impact}. In fuse sacrificing scheme, a fuse picks up a lateral fault before its upstream recloser; whereas in fuse saving scheme, a recloser first attempts to clear the fault by fast tripping. If the fault still persists, it is a permanent fault and is cleared up by the lateral fuse. In case the fault is located between the fuse and recloser, the recloser takes another slow trip after a fuse blown. Most recloser-fuse pairs are coordinated under fuse saving scheme. As shown in Fig.~\ref{fig: fr1},  a recloser's fast tripping curve is  coordinated with a fuse's Minimum Melting (MM) curve, and its slow tripping curve is coordinated with a fuse's Total Clearing (TC) time. In practice, a reclosing sequence takes various form, for example, one fast two slow (F-F-S) or two fast two slow (F-F-S-S) \cite{anderson, Chaitusaney, Girgis, Fazanehrafat}. 

\vspace{-2mm} 
\subsection{DG's impact on coordination and solutions}
In an active distribution grid, fault currents could flow from multiple directions. Hence, reclosers and relays must be retrofit with directional schemes to retrieve coordination \cite{Barker, Girgis}. Since fuses cannot sense currents' direction, if a large amount of DG are connected to laterals, fuse-fuse coordination cannot be retrieved. In this case, fuse needs to be replaced with more advanced protective devices \cite{Fumilayo}. In this paper, we do not attempt to retrieve fuse-fuse coordination and assume DG's are mainly integrated on feeders.    

\subsubsection{Fuse-recloser coordination}
In addition to fault current direction, connecting DG on feeders may disrupt fuse-recloser coordination in two ways: (i) increasing the maximum fault current on feeders; (ii) causing a fault current disparity seen by a coordinated pair \cite{Girgis, Brahma}. In the first case, DG's fault current contribution makes the fault current seen by the fuse exceeding the coordination range. The fault current seen by the recloser and fuse are the same, $I^f_{R,j}=I^f_{F,j}$. Coordination condition \eqref{cod_range} fails if \[I^f_{R,j}+\Delta I^f_{FR,j} > I^f_{max}.\]

%However, the increased fault current exceeds the intersection of the %recloser and fuse's Time Current Inverse (TCI) curve.  
In the second case, DG's fault current contribution makes the fuse response time falling out of the coordination margin. Coordination condition \eqref{cod_margin} fails if \[T_{R,j}(I^f_{max}) < T_{F,i}(I^f_{max} + \Delta I^f_{FR,j}).\]  
%As shown Fig.~\ref{fig: fr2} , the fuse sees more fault current than the recloser, $I^f_{F,j}=I^f_{R,j}+\Delta I^f_{FR,j}$. 

%
%\begin{figure}[t!]
%\vspace{-3mm}
%\setlength{\abovecaptionskip}{-10 pt}
%\hspace*{-5mm}
%\includegraphics[width=0.52\textwidth]{fr2}
%\centering
%\caption{Fuse-recloser coordination margin lost due to installation of DG.}
%\label{fig: fr2}
%\vspace{-4mm}
%\end{figure}

In either case, $I^f_{max}$ for the fuse is increased due to DG's fault current contribution. This fault current increment disrupts the coordination between a recloser' fast tripping curves and a fuse's MM curve. Certainly, DG's fault current contribution also lead to increased $I^f_{min}$. However, this change still will not disrupt the coordination between a recloser's slow tripping curves and a fuse's TC curve. 
\subsubsection{Recloser-recloser coordination}
DG's penetration is unlikely to disrupt recloser-recloser coordination \cite{Abdelaziz}. However, DG's fault current contribution could delay the response from the backup recloser.  Fig.~\ref{fig: rr1} illustrates this effect. For a pair of reclosers with DG units connected to the feeder section in between, the primary recloser sees more fault current, $I^f_{R,j}=I^f_{R,j-1}+\Delta I^f_{RR,j}$, and responses faster. The backup time delay is increased by \[T_{R,j-1}(I^f_{R,j-1}+\Delta I^f_{RR,j})-T_{R,j-1}(I^f_{R,j-1}).\] (The coordination margin is enlarged by $T_{R,j-1}(I^f_{max}+\Delta I^f_{RR,j})-T_{R,j-1}(I^f_{max})$. Hence, coordination condition \eqref{cod_margin} always holds.) With more DG penetrated, this backup delay could become large. Late backup actions will cause damage to equipment. 

\begin{figure}[t!]
\vspace{-3mm}
\setlength{\abovecaptionskip}{-10 pt}
\hspace*{-6mm}
\includegraphics[width=0.53\textwidth]{fr3}
\centering
%\vspace{-4mm}
\caption{Retrieving fuse-recloser coordination by adapting recloser's fast curve. After DG's installation, the fuse picks up the fault current before the recloser. It is observed at maximum fault current, $(T_R-T_F)^0>0$. By adapting the recloser fast tripping curve to DG's fault current contribution ${\Delta} I^f_{FR}$, the recloser picks up the fault before the fuse, $(T_R-T_F)^0<0$. }
\label{fig: fr3}
\vspace{-4mm}
\end{figure} 

\subsubsection{Deficiencies of existing adaptive protection methods}
The solution to the above problems depends on two factors: DG's fault current contribution $I^f_G$ and protective devices' TCI curves. 

A few solutions by adjusting the recloser/relay's TCI curves are proposed in previous studies \cite{Abdelaziz, Chaitusaney, Brahma}. According to the anti-islanding requirements, DG must be disconnected on detection of abnormalities in system operation \cite{basso2004ieee}. The required time for DG to be disconnected varies from a few cycles to 5 seconds \cite{kumpulainen2004analysis, de2012impact}. Based on the current anti-islanding practice, it is common to assume that DG's are disconnected after the first trip of reclosers \cite{Brahma, Chaitusaney, Barker}.

Therefore, to retrieve fuse-recloser coordination, we only need to coordinate a recloser's first tripping curve and a fuse's MM curve. The recloser's first fast curve should be moved downward until the coordination range and coordination margin are restored, as shown in Fig.~\ref{fig: fr3}.

To reduce extra backup delay among reclosers, the TCI curves of the backup recloser is moved downward until the coordination margin is reached, as shown in Fig.~\ref{fig: rr2}. In radial distribution systems, an upstream recloser backups all its downstream devices \cite{Abdelaziz, Brahma}.  

\begin{figure}[t!]
\vspace{-3mm}
\setlength{\abovecaptionskip}{-3 pt}
\hspace*{-3mm}
\includegraphics[width=0.52\textwidth]{rr2}
\centering
\caption{Reducing backup delays between reclosers. By adapting Recloser $j$. The backup delay is restored to $(T_{R,j}-T_{R,j+1})^2$, which is the same as the backup delay before DG's installation$(T_{R,j}-T_{R,j+1})^0$.}
\label{fig: rr2}
\vspace{-1mm}
\end{figure}

Existing solutions can address the protection problem under limited DG penetration. However, at high DG penetration level, solely adjusting recloser/relays' settings will not be sufficient to retrieve protection coordination. An example is illustrated by Fig.~\ref{fig: adplimit}. The fuse-recloser coordination is disrupted due to a large fault current contribution from DG. Shifting down the TCI curve of Recloser $j$ will restore the coordination margin between the fuse and recloser, but it will consequently interferes with the coordination margin between Recloser $j$ and Recloser $j+1$. This problem cannot be solved by adjusting other TCI curves, because the fuse's TCI curve is inflexible to be adjusted, and the downstream Recloser $j+1$ might have reached its minimum time setting.   

\begin{figure}[t!]
\vspace{-3mm}
\setlength{\abovecaptionskip}{-3 pt}
\hspace*{-3mm}
\includegraphics[width=0.49\textwidth]{adplimit}
\centering
\caption{Limitation of existing solutions to retrieving protection coordination. Coordination is lost after DG's installation, $(T_R)^1> (T_F)^1$. By adapting recloser $j$, coordination can be retrieved between recloser $j$ and the fuse, $(T_F-T_R)^2 < {\Delta}T_{FR}$. However, recloser-recloser's coordination margin is interfered, $(T_{R,j}-T_{R,j+1})^2 <{\Delta} T_{RR}$}
\label{fig: adplimit}
\vspace{-4mm}
\end{figure}
 
%Coordination between reclosers is realized by setting their responding time. To minimize areas of service interruption, the recloser at the nearest upstream to the fault operates first, if fails, then is backup by its next upstream recloser. The Time-Current (TC) characteristics of overcurrent reclosers can be classified, by inverse level, as definite, inverse, very inverse, and extremely inverse, depicted in Fig.~\ref{fig: Fig3}. While the definite time reclosers have an almost constant time of response for any current exceeding about 10 times minimum pickup, the extremely inverse reclosers trip much faster at a high fault current. The inverse and very inverse performance are in between. 




%These TC characteristics make the definite time reclosers a good choice for LV networks connected with DG, which intermittency results in a large difference of fault current at its maximum and minimum. However, extreme inverse reclosers display much better features of coordination margins between adjacent reclosers and fuses, especially when there is a considerable drop in fault current from one recloser location to the next, which is often observed in the DG-connected LV networks. Using adaptive reclosers can resolve this choice dilemma: reclosers' Time-Dial Settings (TDS) are adapted to detect fault currents at varying DG's output, in the meanwhile, more inverse TC characteristics are adopted for higher selectivity.




==> submission pdf latex/section2_1.tex <==
Conventional distribution grids are radial in nature, so that faults can be isolated conveniently from its upstream networks. Fig.~\ref{fig: Fig2} shows a typical protection configuration. Before DG's integration, fault current is fed from the single source and decreases along the feeder, flowing to the fault location \textcolor{red}{cite}. Because fault location and severity can be implied from current magnitudes, Over-Current (OC) scheme is deployed to protect the network. The main feeders are protected by reclosers and relays. A distribution network are usually equipped a few reclosers along the feeders, and one relay at the head of the feeders. Along a main feeder, three-phase, two-phase and single-phase laterals are tapped to supply loads. Laterals are protected by fuses. Under distribution automation, some laterals are installed with reclosers (referred in industry as ``trip savers'')\textcolor{red}{cite}. However, the large number of laterals and high cost of lateral reclosers make the fuses, which have much lower cost and less application complicacy, still the top choice for lateral protection. 

\begin{figure}[!t]
\centering
\includegraphics[width=0.48\textwidth]{Fig2}
\caption{Protection configuration of a LV network.}
\label{fig: Fig2}
\vspace{-4mm}
\end{figure}

On the occurrence of a fault, if the primary protective device always picks up before the backup devices, and the backup devices pick up within a required time in case the primary device subject to a failure, then the protection system is said coordinated. For feeder protection, coordination is required among (i) fuse-fuse; (ii) fuse-recloser, (iii) recloser-recloser. The last category includes recloser-relay. 

Protection coordination directly affects system reliability. ~\ref{fig:Fig2} shows two examples. For a fault happens at A, if coordination is lost between two fuses, F1 and F2, F1 will clear the fault before F2, and more customers will be interrupted than necessary. For a temporary fault happens at B, if coordination is lost between a recloser and a fuse, R1 and F3, F3 will blow before R1 trips. Because replacing the fuse is likely to take longer time than reclosing, this loss of coordination converts a temporary fault to permanent fault. The first example results in greater Energy Not Supplied (ENS), and the second results in greater System Average Interruption Duration Index (SAIDI).     

Two concepts to define coordination performance are \it{coordination range} and \it{coordination margin}. For the  
\subsection{protection coordination requirements}

These overcurrent devices operate coordinately to clear faults. Over 95\% of faults in distribution networks are temporary and can be cleared through reclosers. When permanent faults occur, opening reclosers for a preset timeframe will not clear the faults, fuses are melt to isolate the laterals. Once a fuse picks up a fault, it cannot be used again. Replacement of used fuses generates cost \cite{anderson}. Therefore, the coordination between fuses and reclosers are stated by the rule of economics. Namely, once a fault is detected, reclosers should operate first, if the fault is not cleared and appears to be permanent, then fuses are ``consumed'' to take the faulted lateral away. For faults happen on the primary feeder and are not temporary, the CB at the substation side is operated to clear the fault by de-energizing the whole feeder. A CB is also likely to have higher operation rating than reclosers, and operates at occurrence of serious faults that cannot be cleared by reclosers.

Coordination between reclosers is realized by setting their responding time. To minimize areas of service interruption, the recloser at the nearest upstream to the fault operates first, if fails, then is backup by its next upstream recloser. The Time-Current (TC) characteristics of overcurrent reclosers can be classified, by inverse level, as definite, inverse, very inverse, and extremely inverse, depicted in Fig.~\ref{fig: Fig3}. While the definite time reclosers have an almost constant time of response for any current exceeding about 10 times minimum pickup, the extremely inverse reclosers trip much faster at a high fault current. The inverse and very inverse performance are in between. 


\begin{figure}[!t]
\centering
\includegraphics[width=0.5\textwidth]{Fig3}
\caption{Time-Current (TC) inverse characteristics of overcurrent reclosers.}
\label{fig: Fig3}
\vspace{-4mm}
\end{figure}

These TC characteristics make the definite time reclosers a good choice for LV networks connected with DG, which intermittency results in a large difference of fault current at its maximum and minimum. However, extreme inverse reclosers display much better features of coordination margins between adjacent reclosers and fuses, especially when there is a considerable drop in fault current from one recloser location to the next, which is often observed in the DG-connected LV networks. Using adaptive reclosers can resolve this choice dilemma: reclosers' Time-Dial Settings (TDS) are adapted to detect fault currents at varying DG's output, in the meanwhile, more inverse TC characteristics are adopted for higher selectivity.




==> submission pdf latex/section3.tex <==
Due to the limitation of recloser/relay's adaptivity, we consider retrieving protection coordination through controlling DG's fault current contribution in active distribution systems. DG's fault current control can be achieved through hardware deployment, such as fault current limiter \cite{tang2005application, El-Khattam}. However, this method requires extra capital investment and lacks of implementation flexibility. An alternative way is to control DG's output power in pre-fault networks, whose principle is reasoned in this section. 
\vspace{-2mm}

\subsection{DG's types} 

There are three major DG types: synchronous generator, asynchronous generator, and inverter-based generator. Their circuits are shown in Fig.~\ref{fig: DGtypes}. 

\begin{figure}[ht!]
\setlength{\abovecaptionskip}{-3 pt}
\centering
\subfigure[Synchronous]{
\hspace{-4mm}
  \includegraphics[width= .2\textwidth]{fig3_A}
  \label{fig:1a}}
\subfigure[Inverter-based]{
  \includegraphics[width= .09\textwidth]{fig3_C}
  \label{fig:8a}}
 \subfigure[Asynchrounous]{
  \includegraphics[width= .35\textwidth]{fig3_B}
  \label{fig:1b}}\\
\caption{The\'venin equivalent circuit for three major DG types}

\label{fig: DGtypes}
\end{figure}

Synchronous DG includes those driven by conventional energy sources and by renewable energies, such as biomass and solar steam systems \cite{nimpitiwan2007fault}. Their fault current contribution depends on the generator's parameters (subtransient and transient reactance) as well as the equivalent pre-fault voltage. 
%Asynchronous and inverter-based DG are mainly driven by renewable energy. 

Asynchronous generators are represented by Type I and Type II wind turbine generators (i.e. squirrel cage generator and wound rotor induction generator) \cite{windpsrc}. Their initial fault response is determined by the pre-fault slip, which is determined by the wind speed and power output before fault happens. This fault current lasts for a few cycles and diminishes.  

Most DG driven by renewable energy sources are inverter-based, such as, Type III and Type IV wind turbine generators (i.e. variable speed double fed generator and induction generator interfaced through a full AC/DC/AC converter), Photo-Voltaic (PV) panels, fuel cells and etc. \cite{hossain2014, Baran}. The inverter control can be current-based or voltage-based. Current-based control is more often used\cite{Plet,haron2012review}. During the fault response, DG unit's peak fault current occurs during the subtransient timeframe and is determined by its pre-fault terminal voltage. If this subtransient fault current is greater than a  threshold ($2-3$ times of a DG unit's rating current), the inverter is turned off and no fault current is flown from DG. After several cycles, the interter clamps the fault current  to a fix value, which is $1.25-2$ times of a DG unit's rating current \cite{Plet, Baran}.
\vspace{-2mm}
\subsection{Relationship between DG's fault current and power output}
In active distribution systems, DG's pre-fault voltage is determined by feeder's load flow. According to the original version of IEEE 1547, DG shall not actively regulate the voltage at its connection point \cite{ieee1547}. In the 2014 amendment, DG is allowed to regulate voltage under approval of the system operator by changes of its real and reactive power \cite{basso2004ieee}. Based on either standard, DG's terminal voltage is dependent of its output power. Therefore, in calculation of network's pre-fault voltages, DG should be modeled as PQ bus rather than PV bus. This is the main difference between the fault analysis in transmission and active distribution systems. DG's pre-fault terminal voltage can be found by solving the load flow on feeders from\cite{ffwu},
\begin{align}\label{distflow}
\begin{split}
P_{i+1}= P_{i} -r_i(P^2_i+Q^2_i)/V^2_i - (P_{D,i} -P_{G,i})\\ 
Q_{i+1}= Q_{i} -x_i(P^2_i+Q^2_i)/V^2_i - (Q_{D,i} -Q_{G,i})
\end{split}
\end{align}  

After $V_i$ is obtained, DG's Th{\'e}venin equivalent voltage and impedance, for synchronous and asynchronous generators, can be calculated from the circuits in Fig.~\ref{fig: DGtypes}. Inverter-based DG is treated as a constant current source. Then DGs' fault current contribution is solved the combined Th{\'e}venin equivalent circuits of the whole distribution network.     
%Settings of reclosers and CB, along with the choice of fuses, should provide protection that is secure, dependable and selective [ref e]. That is, the protective devices should be able to distinguish fault current from load flow at peak demand time; once a fault happens, they should trip in a way as fast as possible, and to interrupt as few loads as possible. The first requirement can be examined for individual devices' settings, in terms of their TC characteristics and pickup currents. Nevertheless, the later requirement is fulfilled by coordinating groups of protective devices in the distribution grid \cite{anderson}. In previous sections, it has been explained that DG's intetmittency will affect pickup settings of protective devices. In this section, we further analyze how DG's integration disrupt the coordination among protective devices. 
%
%Coordination among the protection devices are classified as (a) fuse to fuse, (b) recloser to fuse, and (c) recloser to recloser~\cite{Girgis}. Despite of its higher operation rating, in coordination study, CB can be treated essentially the same as reclosers \cite{anderson}. It has been shown that coordination can be retained for case (a), only if DG is connected at primary feeders; for case (b) and (c), if reclosers are directional and look only to their downstream~\cite{Brahma},~\cite{Girgis}. Fig.~\ref{fig: Fig2} illustrates these facts: 
%
%i) In conventional LV networks, F1 and F2 are coordinated so that F1 backups F2 for the fault to F2's downstream. When a DG unit is connected between F1 and F2, consider a fault happens to F1's upstream, a dependable operation will be F1 trips and clear the fault path. However, if DG's output is not very high and the time-delay between F1 and F2 is long, F2 may trip before F1. This mis-coordination cannot be fixed, considering there may be faults at both F1's upstream and F2's downstream. 
%
%ii) If overcurrent reclosers are non-directional, tripping by fault currents from both sides of their locations, mis-coordination between reclosers will happen in the same way as described in i). 
%
%Therefore, we presume the conditions in previous studies, that DG's are only connected to main feeders, and overcurrent reclosers are directional. Then, the coordination conditions for (b) recloser to fuse and (c) recloser to recloser, can be formulated by the fault current contribution from DG's, as illustrated by Fig.~\ref{fig: Fig4}. 
%\begin{figure}[!t]
%\centering
%\includegraphics[width=0.48\textwidth]{Fig4}
%\caption{DG's connected to main feeder.}
%\label{fig: Fig4}
%\vspace{-4mm}
%\end{figure}
%\subsection{DG's contribution to fault current disparity}


%In passive radial distribution grids, fault current can only be picked up by its downstream protective devices. In active distribution grids, the same principle holds when reclosers and relays are directional. 
%For a lateral fault downstream to bus $j$, without DG in the distribution grid, the same fault current, $I_{R,j}^f$, is seen by the recloser at $j$ and the fuse at the faulted lateral. According to the TC curves in Fig.~\ref{fig: Fig5}, the recloser trips before the fuse melts, assuming a fault is temporary and saving the fuse~\cite{Girgis},~\cite{anderson}. The recloser may operate a few times, based on its setting. By coordinating the reclosers' first operations, we can ensure the coordination of their later operations. Therefore, only fast TC curves, presenting the reclosers' first operation characteristics, are depicted in the Fig.~\ref{fig: Fig5}.
%\subsubsection{Fuse-recloser fault current disparity} 
Directional recloser/relays only pick up fault currents from their upstream. Given that DG is only connected to feeders, lateral fuses are downstream to all DG units. During a fault, a fuse sees the fault current from all DG units and the substation. The recloser to be coordinated with the fuse at node $j$ only sees fault current from the substation and DG upstream. The fault current disparity between the fuse and recloser is contributed from all DG units downstream node $j$, expressed as   
%When DG is connected to the distribution grid, for the lateral fault downstream to bus $j$, its responsible fuse sees a fault current $I_F^f$, and the recloser at bus $j$ sees a fault current $I_{R,j}^f$. The increased fault current seen by the fuses is attributed to the all DG's connected to the main feeder from bus $j$ until the last bus $n$, and is expressed as:
\begin{equation} \label{eq:recfusedisp}
\Delta I_{FR,j} = \sum_{i\in\mathcal{I}^u_j} I^f_{G,i} .
\end{equation}  
%\subsubsection{Recloser-recloser fault current disparity}

Fault current disparity between Recloser $j$ and Recloser $j+1$ is determined by the fault current contribution from the DG on the section between node $j$ and $j+1$, expressed as:     
\begin{equation} \label{eq:recrecdisp}
I_{RR,j}^\Delta = \sum_{i \in\mathcal{I}^j} I_{G,i}^f .
\end{equation}



%\noindent This disparity is identical for every pair of fuse-recloser in an active distribution system.
%
%
%
%Consequently, the backup time-delay increases to $T_1$. In other words, DG's integration will increase coordination margin among reclosers and will reduce fault clearing time of the protective system. ~\cite{Brahma},~\cite{Girgis}. 


%\begin{figure}[!t]
%\centering
%\includegraphics[width=0.52\textwidth]{Fig5}
%% where an .eps filename suffix will be assumed under latex, 
%% and a .pdf suffix will be assumed for pdflatex; or what has been declared
%\caption{Time-Current Inverse (TCI) curve of reclosers at bus $j$ and bus $j-1$, and of a fuse at a lateral tapped from the section between bus $j$ and bus $j+1$. The fuse TCI curve are shown as a band, starting from the Minimum Melting (MM) time to Total Clearing (TC) time.}
%\label{fig: Fig5}
%\vspace{-4mm}
%\end{figure}
%

%For any lateral fault, responsive fuses see fault current contributed from all power sources in the distribution grid. 
%
%\begin{equation} \label{eq:fusefaultcurr}
%I_F^f = \sum_{i\in\mathcal{I}_0}^{\mathcal{I}_n} I_{G,i}^f ,
%\end{equation}
%
%where $n$ is the last node of the primary feeder, $I_{G,0}^f$ is current fed from the substation. Since \eqref{eq:fusefaultcurr} is true for all fuses regardless of which laterals they are located, choice of fuses should depend on DG's total output, and are not affected by output of individual DG units. 


==> submission pdf latex/section4.tex <==
%The mathematical structure of the proposed protection methods embodies the following benefits: (i) guaranteeing both the economic objective (maximizing total power output from DG's) and protection objective (retaining protection coordination and sensitivity); (ii) reducing computation effort by removing the non-linearity of Time-Current (TC) characteristics of protective devices; (iii) providing application flexibility based on available communication and automation level of distribution grids. 
In this section, we propose a new protection method that simultaneously adjusts recloser/relays' setting and DG's output power in pre-fault networks. The proposed method contains two objectives, minimum delay of backup protective devices and maximum DGs' total output power. The challenge of solving the optimization problem arises from the high non-linearity of recloser/relays' TCI inverse curves. An algorithm is proposed to address this challenge.  
%\begin{itemized}
%\item DGs are mainly connected on feeders. Only few DGs are connected on laterals; 
%\item Recloser and relays are microprocessor based; 
%\item DGs are disconnected from the grid after recloser's first trip. 
%\end{itemized}

%The proposed scheme is formulated as two optimization problems, coupling through a common constraint. This decomposed structure effectively reduces the computation size and complexity of the problem.  
\vspace{-2mm}
\subsection{Formulation}
The first objective is to minimize backup delay for each pair of reclosers. For reclosers on the same feeder, theri TCI curves have similar shapes. Therefore, the reclosers' coordination can be visualized by stacking the TCI curves of all recloser/relays from the one at the feeder's end to that at the feeder's head. Therefore, a minimum total clearing time must lead to minimum backup delay for each pair \cite{anderson}~\cite{Abdelaziz}. The objective is equivalent to, 

\begin{equation} \label{eq:mincleartime}
%\min \sum_{\mathcal J} T_{R,j}(I_{p,j},{TD}_j,I^f_{R,j}) ,
\min \sum_{\mathcal J} T_{R,j}
\end{equation} 

The second objective is to maximize DG's output, 

\begin{equation} \label{eq:maxDG}
\max \sum_{\mathcal{I}} P_{G,i} ,
\end{equation}

%The decision variables under this objective are the pickup current $I^p_{R,j}$ and Time-Dial Setting (TDS) $TD_j$. TC characteristics are highly non-linear, and can be expressed as: 

The two objectives, \eqref{eq:mincleartime} and \eqref{eq:maxDG} are bounded by the protection coordination conditions \eqref{cod_range} and \eqref{cod_margin}. For fuse-recloser and recloser-recloser coordinations, these conditions are specified as, 
%\noindent \begin{enumerate}[i)]
%\item {\it Coordination margin fuse and recloser}
\begin{equation} \label{eq:fusereccoor}
T_{F,j} - T_{R,j} \geq \Delta T_{FR},
\end{equation}
%%where $T_{F,j}$ is the fault clearing time of fuse at laterals that are tapped on the feeder section between bus $j$ and $j+1$; $T_{FR}^\Delta$ is the required delay between operations of the fuse and recloser.
%\item {\it Operation speed requirement between the primary and backup reclosers}
\begin{equation} \label{eq:recreccoor}
T_{R,(j-1)} - T_{R,j} \geq \Delta T_{RR}.
\end{equation}

%where $T_{RR}^\Delta$ is the required delay between operations of the reclosers.
%\end{enumerate}
%Both \eqref{eq:fusereccoor} and \eqref{eq:recreccoor} can be expanded in the form of \eqref{eq:TCchar}, as functions of $I_{p,j}$ and  $TD_j$.

Since the reclosing sequence could contain more than one fast tripping curve, \eqref{eq:fusereccoor} and \eqref{eq:recreccoor} are applied according to the anti-islanding requirements and DG's protection settings. If DG is disconnected from the grid after the recloser's first trip, then \eqref{eq:mincleartime} only coordinates recloser's first fast tripping curve and fuse's MM curve, and \eqref{eq:maxDG} coordinates two reclosers' first fast tripping curves.  

The TCI curve for recloser/relays is specified by \cite{anderson}, 
\begin{equation}\label{eq:TCchar}
T_{R,j} = \frac{a\cdot D_{R,j}}{\left(\frac{I_{R,j}^f}{I^p_{R,j}}\right)^m - c}+b\cdot D_{R,j}+K ,
\end{equation} 
where  $a,b,c,m,$ and $K$ are constants provided by manufactures. 

%The fault current seen by the recloser $I_{R,j}^f$ depends on DG's output power, and can be solved by the procedure presented in Section III.

%An unstated constraint is the fault current in the distribution grid should be within the protective devices' ratings and interrupting capability. 

%It should also be noticed that, because the last recloser is set to respond fastest, its TCI curve is set with lowest ${D}_{R,j}$. Therefore, protection coordination downstream the last recloser can only be retrieved by controlling DGs' power output. 



%where $\{i | i \in \tilde{I}\}$ indicates the DG units authorized to be controlled. This set may naturally exclude some DG types, such as renewables. The objective function is bounded by two constraints:
%\begin{enumerate}[i)]
%\item Coordination requirement between the fuse and recloser;
%\item Maximum fault current for fuses. 
%\end{enumerate}
\vspace{-2mm}
\subsection{Algorithm}
%Formulation of the two constraints, as \eqref{eq:recfusedisp} and \eqref{eq:fusefaultcurr}, has been explained in Section II. Under given settings of protective devices, the first constraint sets the maximum DG output downstream to every recloser; while the second constraint sets the total maximum DG output in the distribution grid.
Equation \eqref{eq:TCchar} is highly nonlinear of the recloser's fault current $I_{R,j}^f$. To reduce the nonlinearity, the formulation is decomposed into two sub-problems, whose objectives are minimizing total fault clearing time and maximizing DG's output. The first sub-problem is constrained by \eqref{eq:fusereccoor} and \eqref{eq:recreccoor}. The second sub-problem is constrained by \eqref{eq:fusereccoor}. To further simplify the second sub-problem, constraint \eqref{eq:fusereccoor} is transformed into a function of DGs' fault current contribution as, 
\begin{equation}\label{eq:fuserecmargin}
\Delta I^f_{FR,j} \leq I^f_{max, F,j} - I^f_{max, R,j} -\Delta I_{FR}
\end{equation}

where $\Delta I_{FR}$ is the current value corresponding to the fuse-recloser coordination margin $\Delta T_{FR}$. Left hand side of \eqref{eq:fuserecmargin} can be obtained from \eqref{eq:recfusedisp}. The maximum fault currents and  $\Delta I_{FR}$ on right hand side are obtained from the first sub-problem. 

%What are the \emph{decision variables} in this sub-problem? The objective function, in \eqref{eq: maxDG}, and the two constraints, in \eqref{eq:recfusedisp} and \eqref{eq:fusefaultcurr}, are functions of the fault currents that are contributed from the controllable DG units. DG's output determines these fault current values, which are derived by solving Thevenin Equivalent of the distribution grid \cite{anderson}. That is to say, DG's output is an implicit function of its fault current. Therefore, in its mathematical essence, the fault current values are the decision variables, even though in system operation it is the DG's output to be controlled. 
%
%The two sub-problems, maximizing DG's output and minimizing total fault clearing time, are coupled through their first constraint, i.e. the coordination condition of fuse-recloser pairs. The decision variables are distinct in the two sub-problems. In other words, the overall optimization problem is completely decomposed. 

Based on the decomposed mathematical structure, we propose an algorithm, illustrated in Fig.~\ref{fig: Fig6}. The two objectives are optimized alternatively. Each sub-problem is optimized after updating the coupling constraints, \eqref{eq:fusereccoor} and \eqref{eq:fuserecmargin}, with the optima obtained from the other problem. By doing so, the non-linearity are extinguished in the first sub-problem, greatly reducing the computation size and complexity.
%
%The initial values may be chosen heuristically or from undergoing conditions. For instance, the first sub-problem can be set as fault current calculated from the prediction of DG's output in next hour. 

The algorithm may start with either sub-problem. For example, the solver starts with the second subproblem, maximizing DGs' output. Initial settings are picked for TCI curves, which implies the maximum fault current in the system. This set of initial values, $(I^p_{R,j},D_{R,j}, I^f_{max, F,j},I^f_{max, R,j})^0$, may be chosen heuristically or from undergoing system operation conditions. The solver calculates for DG's optimal output power $(P_G,i)^1$. With this value, reclosers' fault current $(I^f_{R,j})^1$ can be found by following the procedure in Section III. Then constraint \eqref{eq:fusereccoor} is updated in the first sub-problem. The solver optimizes the total clearing time is minimized and obtains optimal recloser/relay settings, $(I^p_{R,j},D_{R,j})^1$. This completes the first iteration. The iterative optimization process ends when the constraints in the sub-problems cannot be relaxed further by controlling DG's output and adjusting recloser settings.

\begin{figure}[!t]
\centering
\includegraphics[width=3in]{Fig6}
\caption{Algorithm for the proposed protection scheme. The decomposed optimization problems are solved alternatively by updating the coupling constraint. The initial value is input as $(.)^0$, the kth iteration is denoted as $(.)^k$.}
\label{fig: Fig6}
\vspace{-4mm}
\end{figure}

\subsection{Implementation and Dependence on Distribution Automation} 
The proposed protection method and algorithm enable implementation flexibility based on system operation conditions. In practice, the frequencies of adapting reclosers and controlling DG depend on a few factors, such as DGs' type and intermittency, authorized intervention to DG's natural output, communication readiness of the grid, and etc. For DG of high intermittency and their fault current highly dependent of power output, such as Type I and II wind turbine generator and solar steam systems, the protection settings could be adapted hourly or more frequently. This flexibility is tested in Section V with practical numerical examples. 
%Based on need, one objective may be optimized more frequently than the other. For example, adapting frequency and accuracy are relaxed for reclosers, if DG's output is controlled in a more restrict manner at shorter time interval. 


The proposed protection method requires metering at all DG locations and remote control of the authorized DG units. Today's distribution grid may not completely fulfill these requirements. The proposed method provides the flexibility to be implemented progressively in accordance with the grid's available automation level. Equation \eqref{eq:recfusedisp} to \eqref{eq:recrecdisp} show that the requirements of metering and communication declines as the protection goals become more critical. For example, for fuses' secure operation, only DG at reclosers' upstream need to be controlled; for minimum backup delay, DG need to be controlled at every feeder section between two reclosers. The later protection goal requires more discrete monitoring and communication, but presents relatively less protection criticalness. This is a favorable characteristic in implementation, in the sense that the most critical protection requirement can be fulfilled at an earlier stage of distribution automation.

%Numerical examples are included in Section V, exploring implementations at different stages in transition to a fully active distribution network. 

==> submission pdf latex/section5.tex <==
This section demonstrates the benefits of the proposed protection scheme with an IEEE 37-bus system. The system configuration is altered with DG integration and shown in Fig.~\ref{fig: system}.  The main feeder is protected with 3 reclosers, which locations are shown in Table~\ref{table:faultcurr}. The proposed protection method, short circuit analysis and power flow were implemented in MATLAB.

\begin{figure}[!t]
\vspace{-3mm}
\centering
\includegraphics[width=0.25\textwidth,angle=90]{Fig10r}
\caption{IEEE 37-bus distribution system with DGs connected in the main feeder.}
\label{fig: system}
\vspace{-4mm}
\end{figure}

In the test system, the reclosers' TCI characteristics are modeled with \eqref{eq:TCchar}. Without losing generality, the reclosers' Time-Dial Setting (TDS) and pickup current are assumed to be continuous. The TDS' are selected from the interval, ${D}_{R,j} \in [0.1,1]$, and the pickup currents $I^p_{R,j}$ are chosen twice greater than the maximum load current and less than 50\% of Line-Line fault current~\cite{anderson}. Fuses' TC characteristics are represented by their minimum melting curves and are linearized ~\cite{anderson}.

The initial settings of the protective devices are based on the configuration without DG's integration. The maximum currents at reclosers' bus are calculated in Table~\ref{table:faultcurr}. The reclosers are set based on the procedure described in Section II. Since R3 only needs to coordinate with its lateral fuse, its TDS can be selected to be the lowest, that is ${D}_{R,3}=0.1$. The rest of the reclosers are coordinated in pairs.  

\begin{table}[ht]
\vspace{-5mm}
\caption{Reclosers' Max/Min Fault Currents}
\centering
\begin{tabular}{|c |c | c |}
\hline 
Recloser & Bus & Max  Fault Current (A) \\ [0.5ex]
\hline
R1 & 702 & 2975   \\ [0.5ex]
\hline
R2 & 709 & 2445   \\ [0.5ex]
\hline
R3 & 711 & 1823   \\ [0.5ex]
\hline
\end{tabular}
\label{table:faultcurr}
\end{table}
\vspace{-5mm}

\subsection*{Case A: Single-step implementation}
The proposed method is tested assuming all DG are controllable and their output known in advance. For a 3-phase fault on Lateral 2, DG's integration will disrupt coordination between the recloser, R2, and fuse, F2, as shown in Fig.~\ref{fig: Fig14r}. Due to the large high penetration level of DG in the systme, coordination cannot be restored by solely adapting R2's TCI curve. With the proposed method, DG's output is controlled to regain the coordination margin. The tripping sequence restoration procedure is illustrated in Fig.~\ref{fig: Fig13r}.


%It can be observed that, without DG in the system, the maximum fault current seen by R2 and the fuse is $I^f_{R,2,\max}$. At this current, R2 trips faster than the fuse, so the coordination is held. The tripping sequence of R2 and F2 is depicted in the top part of Fig.~\ref{fig: Fig13r}. After DG2 is connected, R2 still sees the same fault current, but F2 sees a fault current $I^{f}_{F,2,\max}$. This fault current disparity leads to F2 tripping faster than R2, namely, $T_F < T^0_{R,2}$. The fuse and recloser coordination is disrupted at this point, as depicted in the middle part of Fig.~\ref{fig: Fig13r}.


\begin{figure}[!t]
\setlength{\abovecaptionskip}{-3 pt}
\centering
\includegraphics[width=0.5\textwidth]{Fig14r}
\caption{TCI curves of R2 and F2. R2 Original and R2 adaptive are the R2's TC curves using basic (non-adaptive) protection and adaptive protection; initial and adapted DG power output.}
\label{fig: Fig14r}
\vspace{-4mm}

\end{figure}



%\begin{figure}[!t]
%\centering
%\includegraphics[width=0.5\textwidth]{Fig11r}
%\caption{Time-Current (TC) curves of R2 and F2 in Fig.~\ref{fig: Fig10r}. R2 Original and R2 adaptive are the R2's TC curves using basic (non-adaptive) protection and adaptive protection, respectively. Fuse is linearized TC characteristics of F2.}
%\label{fig: Fig11r}
%\vspace{-4mm}
%\end{figure}

Reclosers' coordination is examined under basic and adaptive protection. Recloser R2 backups R3 for a fault on Lateral 3. Fig.~\ref{fig: Fig12r} shows that, before DG's integration, the backup time interval between R2 and R3 is $T_0 = (T_{R,2}-T_{R,3})^0$. DG2's connection increase the maximum fault current seen by R3 as $I^{f}_{R,3,\max}$. The resultant delay between R2 and R3 is increased to $T_1 = (T_{R,2}-T_{R,3})^1$ and $T_0 < T_1$. To reduce this backup clearing time, R2 is adapted to reduce the backup fault clearing time to $T_2 = (T_{R,2}-T_{R,3})^2$.

%This observation provides intuition for the first sub-problem in Section IV: connecting DG between reclosers will increase the backup fault clearing time, while adapting the recloser settings can reduce the fault clearing time to less than before DG's connection. In other words, DG's integration can improve the security of protective devices in a distribution grid. 

\begin{figure}[!t]
\setlength{\abovecaptionskip}{-3 pt}
\centering
\includegraphics[width=0.5\textwidth]{Fig12r}
\caption{TCI curves of R2 and R3.R2 Original and R2 adaptive are the R2's TC curves using basic (non-adaptive) protection and adaptive protection, respectively. }
\label{fig: Fig12r}
\vspace{-4mm}
\end{figure}

\begin{figure}[!t]
\setlength{\abovecaptionskip}{-3 pt}
\centering
\includegraphics[width=0.5\textwidth, height=7cm]{Fig13r}
\caption{Tripping sequence of F2 and R2 in Fig.~\ref{fig: system}. Top: no DG is connected in the test system; Middle: with DG integrated and basic (non-adaptive) protection; Bottom: with DG integrated and conventional adaptive protection}
\label{fig: Fig13r}
\vspace{-4mm}
\end{figure}



%\subsection*{Case B: Accommodating DG of time-varying output}
%The proposed method is tested on the system integrated with renewable energy sources. With no DG in the system, with a total fault clearing time of, $\sum T_{R,j} = 2.05 [s]$.
%
%Since renewable energy sources are not controllable, the proposed protection scheme is only active in its first sub-problem, namely, minimizing total fault clearing time. The main results are displayed as time-series in Fig.~\ref{fig: Fig15r}. The reclosers are adapted at every hours. For conciseness, only R2's TDS is shown to demonstrate the adapting procedure. It can be observed that the total fault clearing time and time dials are reduced drastically in the first step. It is because DG are set offline at time zero. After DG starting to inject power into the system, the fault current allocation is changed for all reclosers, activating the proposed protection scheme. The total fault clearing time is reduced at higher DG's output. When DG's output falls down, the coordination margin between reclosers are reduced, and recloser's TDS is pushed back, according to \eqref{eq:recreccoor}, for secure operations. 
%
%\begin{figure}
%\setlength{\abovecaptionskip}{-3 pt}
%\centering
%\includegraphics[width=0.5\textwidth]{Fig15r}
%% where an .eps filename suffix will be assumed under latex, 
%% and a .pdf suffix will be assumed for pdflatex; or what has been declared
%\caption{Proposed protection scheme under renewable DG integration. The test system is shown in Fig.~\ref{fig: system}. (a) Renewable DG output; (b) Time-Dial Setting of R2; (c) total fault clearing time of all reclosers.}
%\label{fig: Fig15r}
%\vspace{-4mm}
%\end{figure}


\subsection*{Case B: Multiple-step implementation }
The benefits of proposed protection method is fully realized when DG of mixed types is integrated to the system. As shown in Fig.~\ref{fig: Fig16r}(a), both inverter-based and controllable DG present in the test system. We demonstrate the flexibility of the proposed scheme by adapting DG's output and recloser settings at one hour and five hours, respectively. This scenario has practical implications, since protective systems are less often adapted and DG, as could be involved in demand response programs, is not rare controlled hourly. 

\begin{figure}[!t]
\setlength{\abovecaptionskip}{-3 pt}
\centering
\includegraphics[width=0.5\textwidth]{Fig16r}
\caption{Proposed protection scheme under DG of mixed types integration. The test system is shown in Fig.~\ref{fig: system}. (a) DG's output; (b) Time-Dial Setting of R2; (c) total fault clearing time of all reclosers.}
\label{fig: Fig16r}
\vspace{-4mm}
\end{figure}

Fig.~\ref{fig: Fig16r} shows that the total DG output is maximized to reduce the fault clearing time in the system. At peak period of renewable generation, the controllable DG units are commanded to produce less power, to ensure recloser and fuse coordination and prevent unnecessary fuse operation, as in \eqref{eq:fusereccoor} and \eqref{eq:recfusedisp}.   
